Green Architectural Tactics in ML-enabled Systems: An LLM-based Repository Mining Study

Context: The increasing adoption of machine learning (ML) and artificial intelligence (AI) technologies raises growing concerns about their environmental sustainability. Developing and deploying ML-enabled systems is computationally intensive, particularly during training and inference. Green AI has emerged to address these issues by promoting efficiency without sacrificing accuracy. While prior research has proposed catalogs of sustainable practices (i.e., green tactics), there remains limited understanding of their adoption in practice and whether additional, undocumented tactics exist. Objective: This study aims to investigate the extent to which existing sustainable practices are implemented in real-world ML-enabled systems and to identify previously undocumented practices that support environmental sustainability. Method: We conduct a mining software repository study on 205 open-source ML projects on GitHub. To support our analysis, we design a novel mechanism based on large language models (LLMs) capable of identifying both known and new sustainable practices from code repositories. Results: Our findings confirm that green tactics reported in the literature are used in practice, although adoption rates vary. Furthermore, our LLM-based approach reveals nine previously undocumented sustainable practices. Each tactic is supported with code examples to aid adoption and integration. Conclusions: We finally provide insights for practitioners seeking to reduce the environmental impact of ML-enabled systems and offer a foundation for future research in automating the detection and adoption of sustainable practices.

==> Abstract.tex <==
\begin{abstract}
As machine learning (ML) and artificial intelligence (AI) technologies become increasingly prevalent in society, concerns about their environmental sustainability have grown. Developing and deploying ML-enabled systems, especially during training and inference, are resource-intensive, raising sustainability issues. Green AI has emerged as a response, advocating for reducing the computational demands of AI while maintaining accuracy. While recent research has identified various green tactics for developing sustainable ML-enabled systems, there is a gap in understanding the extent to which these tactics are adopted in real-world projects and whether additional, undocumented practices exist. This paper addresses these gaps by presenting a mining software repository study that evaluates the adoption of green tactics in 168 open-source ML projects on \textsc{GitHub}. In doing so, we introduce a novel mining mechanism based on large language models to identify and analyze green tactics within software repositories. Our results provide insights into the adoption of green tactics found in the literature and expand previous catalogs by providing 12 new tactics, with code examples to support wider implementation. This study contributes to the development of more sustainable ML systems by identifying adopted green tactics that offer substantial environmental benefits with minimal implementation effort. It provides practical insights for developers to green their systems and offers a path for future research to automate the integration of these tactics.
\end{abstract}

==> size_metrics.tex <==

\begin{table*}[t]
\caption{Metrics for Different Sizes of Projects}
\centering
\footnotesize
    \begin{tabular}{|l|c|c|c|c|c|c|c|}
    \rowcolor{black}
    {\textcolor{white} {\textbf{Size}}} & {\textcolor{white} {\textbf{Number Project}}} & {\textcolor{white} {\textbf{Median Age}}} & {\textcolor{white} {\textbf{Median Stars}}} & {\textcolor{white} {\textbf{Median Size}}} & {\textcolor{white} {\textbf{Median Contributors}}} & {\textcolor{white} {\textbf{Median Forks}}} & {\textcolor{white} {\textbf{Median Commit}}} \\
    \hline
    Small & 17 & 5.7 & 157 & 244 & 3 & 44 & 95\\
    \hline
    Medium & 102 & 6.25 & 630 & 16789.5 & 9 & 131.5 & 577\\
    \hline
    Large & 49 & 6.6 & 563 & 248857 & 21 & 154 & 1506\\
    \hline
    \end{tabular}
\label{table:size_project_metrics}
\end{table*}
